Efficient Full-Matrix Adaptive Regularization

Adaptive regularization methods pre-multiply a descent direction by a preconditioning matrix. Due to the large number of parameters of machine learning problems, full-matrix preconditioning methods are prohibitively expensive. We show how to modify full-matrix adaptive regularization in order to make it practical and effective. We also provide a novel theoretical analysis for adaptive regularization in non-convex optimization settings. The core of our algorithm, termed GGT, consists of the efficient computation of the inverse square root of a low-rank matrix. Our preliminary experiments show improved iteration-wise convergence rates across synthetic tasks and standard deep learning benchmarks, and that the more carefully-preconditioned steps sometimes lead to a better solution.

==> epoched_adagrad.tex <==
%auto-ignore
%!TEX root=main-appendix.tex

%\paragraph{Proof of Theorem \ref{thm:reduction}}
\begin{proof}[Proof of Theorem \ref{thm:reduction}]
  From the statement of the theorem we have that 
  \[f_t(x_{t+1}) - f_t(\argmin_{x\in \mathcal{K}} f_t(x)) \leq \Gamma(f_t, T')\]
  Now consider the following equations which hold for any $t$ and any $\eta > 0$. 
  \begin{align*}
    f(x_t) - f(x_{t+1}) &\geq f(x_t) - f_t(x_{t+1}) \\
    &= f(x_t) - f_t(\argmin_{x\in \mathcal{K}} f_t(x)) +  f_t(\argmin_x f_t(x)) - f_t(x_{t+1}) \\
    &\geq f(x_t) - f_t(x_t - \eta \nabla f(x_t)) - \Gamma(f_t, T') \\ 
    &= f(x_t) - f(x_t - \eta \nabla f(x_t)) - \frac{3L\eta^2}{2} \|\nabla f(x_t)\|^2 - \Gamma(f_t, T') \\
    &\geq \eta \|\nabla f(x)\|^2 - 2L\eta^2 \|\nabla f(x)\|^2 - \Gamma(f_t, T'),
  \end{align*}
  where the last inequality follows from smoothness.
  Now setting $\eta = 1/4L$, summing the inequality over $t$ and rearranging gives us that
  \[ \frac{1}{T}\sum_{t = 1}^T\|\nabla f(x_t)\|^2 \leq \frac{8L}{T} \sum_{t=1}^T \left(f(x_t) - f(x_{t+1}) + \Gamma(f_t, T') \right) \leq \frac{8L}{T} \left(M + \sum_{t = 1}^{T} \Gamma(f_t, T') \right) \] 
  which proves the theorem.
\end{proof}

%\paragraph{Proof of Theorem \ref{thm:sc_ag}}

\begin{proof}[Proof of Theorem \ref{thm:sc_ag}]
Define $V_1 = M, V_{i+1}  = \frac{V_i}{2}, i = 1, \ldots, N$. The first claim is that at the end of each epoch $i$, it holds that
\[ \E [ f(x_i^0) ] - f(x^*) \leq V_i.\]
Note that the claim is true for $i=1$ as $V_1=M$.

Additionally, for any epoch $i$ we have
\begin{align*}
  \E\bra{ f(x_{i+1}^0) } - f(x^*) &\leq \frac{1}{T'} \sum_{t=1}^{T'} \E [f(x_i^t)] - f(x^*) \leq\frac{1}{T'} \mathbb{E} \bra{ \sum\limits_{t=1}^{T'} \nabla f(x_i^t)^\top (x_i^t - x^*) }\\
  &= \frac{1}{T'} \E \bra{ \sum_{t=1}^{T'} (g_i^t)^\top (x_i^t -x^*) } \leq \E\bra{ \frac{\mu \sqrt{\sum_{t=1}^{T'}\|g_i^t\|^2}}{T'} \|x_i^0 - x^*\| } \\
  &\leq \E \bra{ \frac{\mu \sigma}{\sqrt{T'}} \|x_i^0 - x^*\| } \leq \E\bra{ \frac{\mu \sigma\sqrt{(f(x_i^0)- f(x^*))}}{\sqrt{LT'}} }\\
\end{align*}
Note that the minimum value of $V_i$ for any $i$ is $\frac{M}{2^{\lceil \log \frac{M}{\eps}\rceil}} \geq \frac{M}{2^{\log \frac{M}{\eps} + 1}} \geq  \frac{\eps}{2}$, so $T \ge \frac{4\mu^2\sigma^2}{V_iL}$. Therefore
\begin{align*}
\E[f(x_{i+1}^0)] - f(x^*) \le \E\bra{ \frac{\sqrt{(f(x_i^0)- f(x^*))}}{2} }\sqrt{V_i} \le \frac{V_i}{2} = V_{i+1}
\end{align*}
where the last inequality is due to the induction hypothesis and Jensen's inequality. As a consequence, we have
\begin{align*}
  \E [f(x)] - f(x^*) \leq \frac{M}{2^{\lceil \log \frac{M}{\eps}\rceil}} \leq \eps
\end{align*}
The total number of stochastic gradient oracle calls the algorithm makes is $ \frac{8\mu^2 \sigma^2}{\eps L} \lceil\log \frac{M}{\eps}\rceil$.
\end{proof}

==> motiv.tex <==
%auto-ignore
%!TEX root=main-appendix.tex

\subsection{Example: the advantage of adaptivity}
\label{sec:example}

This section shows an example originally provided in \cite{duchi2011adaptive}, where the constant of adaptivity for full matrix AdaGrad is much smaller than 1 and adaptive regularization methods have  significant advantage over SGD. Consider the setting where in each iteration we receive a training example $z_t \in \R^d$ and suffer hinge loss $f_t(x) = \lbrack 1 - y_t \langle x, z_t\rangle\rbrack_{+}$. Let $V$ be an orthonormal matrix and $v_i$ denote its columns. Let $y_t = \text{sign}(\langle \mathbf{1}, V^\top z_t\rangle)$ and our domain be $\cK=\{x: \|x\|_2 \le \sqrt{d}\}$, then $x^* = \sum\limits_{i=1}^d v_i \in \cK$ is an optimum. Suppose for a fixed $T$, we receive examples in the following way:
\[
     z_t = \begin{cases}
        v_1, & \text{for } t = 1, \dots, \frac{T}{d}\\
        \vdots\\
        v_d, & \text{for } t = \frac{T(d-1) + 1}{d}, \dots, T
        \end{cases}
\]
We show that in this case $\mu \ll 1$.  
We initialize $x_0 = 0$. After the first iteration, AdaGrad updates $x_{1} = (v_1 v_1^\top)^{-1/2} v_1 = v_1$ and we have zero loss until the algorithm sees $v_2$. Since $v_1$ and $v_2$ are orthogonal, $x_{\frac{T+1}{d}} = v_1 + v_2 \in \cK$. Similarly, AdaGrad suffers constant loss in each dimension, and $\mu = \frac{d}{\|x_0 - x^*\|_2 \sqrt{T}} = \sqrt{\frac{d}{T}}\ll 1$. 
